Exploring Semantic Masked Autoencoder for Self-supervised Point Cloud Understanding

Point cloud understanding aims to acquire robust and general feature representations from unlabeled data. Masked point modeling-based methods have recently shown significant performance across various downstream tasks. These pre-training methods rely on random masking strategies to establish the perception of point clouds by restoring corrupted point cloud inputs, which leads to the failure of capturing reasonable semantic relationships by the self-supervised models. To address this issue, we propose Semantic Masked Autoencoder, which comprises two main components: a prototype-based component semantic modeling module and a component semantic-enhanced masking strategy. Specifically, in the component semantic modeling module, we design a component semantic guidance mechanism to direct a set of learnable prototypes in capturing the semantics of different components from objects. Leveraging these prototypes, we develop a component semantic-enhanced masking strategy that addresses the limitations of random masking in effectively covering complete component structures. Furthermore, we introduce a component semantic-enhanced prompt-tuning strategy, which further leverages these prototypes to improve the performance of pre-trained models in downstream tasks. Extensive experiments conducted on datasets such as ScanObjectNN, ModelNet40, and ShapeNetPart demonstrate the effectiveness of our proposed modules.

==> table.tex <==
\begin{table*}[!t]
  % \vspace{-0.5em}
  \begin{center}
    % \setlength\tabcolsep{7pt}
    \caption{\textbf{Shape Classification on ScanObjectNN and ModelNet40 Datasets.} For ScanObjectNN dataset, we report the classification accuracy(\%) over the three subsets: OBJ-BG, OBJ-ONLY and the most challenging variant PB-T50-RS. For ModelNet40 dataset, we report the linear SVM evaluation as well as the finetuning results with and without the voting trick.
    %
    The gray part represents methods that use cross-modal information or extra pre-training data.}
    \small
    \label{table:ScanObjectNN}
    % \vspace{-0.8em}
    \begin{tabular}{l|ccc||ccc}
      \toprule
      % \hline
      \multirow{2}*{Method}               & \multicolumn{3}{c||}{ScanObjectNN} & \multicolumn{3}{c}{MODELNET40}                                                                                         \\
      \cline{2-7}
      ~                                   & $\mbox{OBJ-BG}$                    & $\mbox{OBJ-ONLY}$              & $\mbox{PB-T50-RS}$  & $\mbox{SVM}$        & $\mbox{w/o Voting}$ & $\mbox{w/ Voting}$  \\
      \midrule
      % \cline{1-11}

      Point-BERT~\cite{yu2022pointbert}   & 87.4                               & 88.1                           & 88.1                & 87.4                & 92.7                & 93.2                \\
      % \cline{1-11}
      MaskPoint~\cite{liu2022maskpoint}   & 89.3                               & 88.1                           & 84.3                & -                   & -                   & 93.8                \\
      Topology3D~\cite{}                  & -                                  & -                              & -                   & 89.6                & -                   & -                   \\
      MAE3D~\cite{jiang2023masked}        & 88.4                               & 87.7                           & 86.2                & -                   & 93.4                & -                   \\
      PointMAE~\cite{pang2022pointmae}    & 90.0                               & 88.3                           & 85.2                & 92.7                & 93.2                & 93.8                \\
      PointGame~\cite{liu2023pointgame}   & 89.0                               & 89.0                           & 85.8                & 90.0                & 93.1                & 93.5                \\
      PointLGMask~\cite{tang2023point}                 & 89.8                               & 89.3                           & 85.3                & -                   & -                   & -                   \\
      PointM2AE~\cite{zhang2022pointm2ae} & 91.2                               & 88.8                           & 86.4                & 92.9                & 93.4                & 94.0                \\
      PointGPT-S~\cite{chen2023pointgpt}  & 91.6                               & 90.0                           & 86.8                & -                   & -                   & 94.2                \\
      \textbf{Ours}                       & \textbf{92.9}                      & \textbf{92.3}                  & \textbf{89.0}       & \textbf{93.4}       & \textbf{94.3}       & \textbf{94.5}       \\
      % \midrule
      % \multicolumn{4}{l}{Methods using cross-modal information or extra training data}                                         \\
      \hline
      CorssNet~\cite{wu2023self}          & {\color{gray} -}                   & {\color{gray} -}               & {\color{gray} -}    & {\color{gray} 91.5} & {\color{gray} 93.4} & {\color{gray} -}    \\
      InterMAE~\cite{liu2023inter}        & {\color{gray} 88.7}                & {\color{gray} 89.6}            & {\color{gray} 85.4} & {\color{gray} -}    & {\color{gray} 93.6} & {\color{gray} -}    \\
      ACT~\cite{dong2023act}              & {\color{gray} 93.3}                & {\color{gray} 91.9}            & {\color{gray} 88.2} & {\color{gray} -}    & {\color{gray} 93.7} & {\color{gray} 94.0} \\
      I2P-MAE~\cite{zhang2023i2pmae}      & {\color{gray} 94.2}                & {\color{gray} 91.6}            & {\color{gray} 90.1} & {\color{gray} -}    & {\color{gray} 93.7} & {\color{gray} 94.1} \\
      ReCon~\cite{qi2023recon}            & {\color{gray} 95.4}                & {\color{gray} 93.6}            & {\color{gray} 91.3} & {\color{gray} -}    & {\color{gray} 94.5} & {\color{gray} 94.7} \\
      PointGPT-L~\cite{chen2023pointgpt}  & {\color{gray} 97.2}                & {\color{gray} 96.6}            & {\color{gray} 93.4} & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} 94.7} \\

      \bottomrule
    \end{tabular}
    % \vspace{-1em}
  \end{center}
  % \vspace{-1em}
\end{table*}


\begin{table*}[!t]
  % \vspace{-0.5em}
  \begin{center}
    % \setlength\tabcolsep{16pt}
    \caption{\textbf{Part Segmentation on ShapeNetPart Dataset.} We report the $\operatorname{mIoU}$ across all part categories ($\operatorname{Cls.}$) and the $\operatorname{mIoU}$ across all instances ($\operatorname{Inst.}$). The gray part represents methods that use cross-modal information or extra pre-training data.}
    \small
    \label{table:ShapeNetPart}
    % \vspace{-0.8em}
    \begin{tabular}{l|cccccccccccccccccc}
      \toprule
      % \hline
      \multirow{1}*{Method}               & $\text{mIoU}_c$     & $\text{mIoU}_i$     & airplane            & bag                 & cap                 & car                 & chair               & earphone            & guitar              \\
      \midrule
      Point-BERT~\cite{yu2022pointbert}   & 84.1                & 85.6                & 84.3                & 84.8                & 88.0                & 79.8                & 91.0                & \textbf{81.7}       & 91.6                \\
      MaskPoint~\cite{liu2022maskpoint}   & 84.4                & 86.0                & 84.2                & 85.6                & 88.1                & 80.3                & 91.2                & 79.5                & 91.9                \\
      MAE3D~\cite{jiang2023masked}        & 82.5                & 85.6                & 83.7                & 81.7                & 85.3                & 78.5                & 90.8                & 80.1                & 91.4                \\
      PointMAE~\cite{yu2022pointbert}     & 84.1                & 86.1                & 84.3                & 85.0                & 88.3                & 80.5                & 91.3                & 78.5                & \underline{92.1}    \\
      PointGame~\cite{liu2023pointgame}                   & 84.2                & 86.1                & 84.8                & 84.5                & 88.7                & 80.7                & 91.3                & 78.6                & \textbf{92.2}       \\
      PointLGMask~\cite{tang2023point}                 & 84.4                & 86.1                & 84.9                & 84.7                & 88.4                & 80.5                & \underline{91.5}    & 78.4                & 92.1
      \\
      PointGPT-S*~\cite{chen2023pointgpt} & 84.0                & 85.9                & \underline{85.1}    & \underline{86.1}    & 88.8                & 80.2                & 91.2                & 78.8                & 91.7                \\
      PointM2AE~\cite{zhang2022pointm2ae} & \underline{84.9}    & \underline{86.5}    & \underline{85.1}    & \textbf{88.0}       & \underline{88.9}    & \textbf{81.3}       & \textbf{91.6}       & 78.8                & 92.0                \\
      \textbf{Ours}                       & \textbf{85.1}       & \textbf{86.8}       & \textbf{85.4}       & 85.9                & \textbf{89.2}       & \underline{80.8}    & 91.4                & \underline{81.6}    & 91.9
      \\
      \hline
      CorssNet~\cite{wu2023self}                    & {\color{gray}82.5}  & {\color{gray}85.5}  & {\color{gray}83.7}  & {\color{gray}78.8}  & {\color{gray}86.8}  & {\color{gray}77.7}  & {\color{gray}91.5}  & {\color{gray}74.0}  & {\color{gray}98.0}
      \\
      InterMAE~\cite{liu2023inter}                    & {\color{gray} 84.3} & {\color{gray} 86.3} & {\color{gray} 84.7} & {\color{gray} 84.8} & {\color{gray} 88.6} & {\color{gray} 81.2} & {\color{gray} 91.5} & {\color{gray} 77.3} & {\color{gray} 92.3} \\

      % ACT~\cite{dong2023act}                       & {\color{gray}84.7}  & {\color{gray} 86.1}                                                                                                                                                                                        \\
      ReCon*~\cite{qi2023recon}           & {\color{gray}84.1}  & {\color{gray}86.3}  & {\color{gray}85.2}  & {\color{gray}85.2}  & {\color{gray}87.2}  & {\color{gray}80.9}  & {\color{gray}91.5}  & {\color{gray}72.5}  & {\color{gray}92.3}
      \\
      I2P-MAE~\cite{zhang2023i2pmae}      & {\color{gray} 85.2} & {\color{gray} 86.8} & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    \\
      \midrule
      \multirow{1}*{Method}               & knife               & lamp                & laptop              & motorbike           & mug                 & pistol              & rocket              & skateboard          & table               \\
      \midrule
      Point-BERT~\cite{yu2022pointbert}   & 87.9                & 85.2                & 95.6                & 75.6                & 94.7                & 84.3                & 63.4                & 76.3                & 81.5
      \\
      MaskPoint~\cite{liu2022maskpoint}   & 87.8                & \underline{86.2}    & 95.3                & 76.9                & \underline{95.0}    & \textbf{85.3}       & 64.4                & 76.9                & 81.8
      \\
      MAE3D~\cite{jiang2023masked}        & \textbf{89.1}       & 84.6                & 95.5                & 66.7                & 94.8                & 81.9                & 58.5                & 74.6                & \underline{82.7}
      \\
      PointMAE~\cite{yu2022pointbert}     & 87.4                & 86.1                & \underline{96.1}    & 75.2                & 94.6                & 84.7                & 63.5                & 77.1                & 82.4
      \\
      PointGame~\cite{}                   & \underline{88.3}    & 85.9                & 95.9                & 75.5                & \underline{95.0}    & \underline{85.1}    & 62.0                & \underline{77.2}    & 82.0
      \\
      PointLGMask~\cite{}                 & 87.5                & 86.0                & 96.0                & \textbf{78.1}       & 94.6                & \underline{85.1}    & 64.4                & 76.4                & 81.8

      \\
      PointGPT-S*~\cite{chen2023pointgpt} & 87.0                & 84.5                & 95.9                & 74.2                & \underline{95.0}    & 83.8                & 62.6                & 76.8                & 81.6
      \\
      PointM2AE~\cite{zhang2022pointm2ae} & 87.9                & 85.7                & 95.9                & \underline{77.9}    & \underline{95.0}    & 84.5                & \textbf{66.3}       & 76.7                & 82.2
      \\
      \textbf{Ours}                       & \textbf{89.1}       & \textbf{86.3}       & \textbf{96.3}       & 76.4                & \textbf{95.5}       & \textbf{85.3}       & \underline{65.3}    & \textbf{77.9}       & \textbf{83.4}
      \\
      \hline
      CorssNet~\cite{}                    & {\color{gray} 88.1} & {\color{gray}84.8}  & {\color{gray}96.3}  & {\color{gray}68.0}  & {\color{gray}93.8}  & {\color{gray}80.9}  & {\color{gray}59.0}  & {\color{gray}75.3}  & {\color{gray}83.1}
      \\
      InterMAE~\cite{}                    & {\color{gray} 87.4} & {\color{gray} 85.3} & {\color{gray} 95.9} & {\color{gray} 76.0} & {\color{gray} 95.0} & {\color{gray} 66.0} & {\color{gray} 76.1} & {\color{gray} 81.6}                       \\
      ReCon*~\cite{qi2023recon}           & {\color{gray}87.4}  & {\color{gray}86.2}  & {\color{gray}96.1}  & {\color{gray}76.9}  & {\color{gray}94.9}  & {\color{gray}85.8}  & {\color{gray}65.0}  & {\color{gray}76.7}  & {\color{gray}82.2}
      \\
      I2P-MAE~\cite{zhang2023i2pmae}      & {\color{gray} 85.2} & {\color{gray} 86.8} & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}    & {\color{gray} -}                          \\



      \bottomrule
    \end{tabular}
    % \vspace{-1em}
  \end{center}
  % \vspace{-1em}
\end{table*}



\begin{table}[!t]
  % \vspace{-0.5em}
  \begin{center}
    \setlength\tabcolsep{5pt}
    \caption{\textbf{Few-Shot Classification on ModelNet40.} We report mean and standard deviation over ten runs in each setting. The gray part represents methods that use cross-modal information or extra pre-training data.}
    % \small
    \label{table:fewshot}
    % \vspace{-0.8em}
    \begin{tabular}{l|cc|cc}
      \toprule
      % \hline
      \multirow{2}*{Model}                & \multicolumn{2}{c|}{5-way}                & \multicolumn{2}{c}{10-way}                                                                                                        \\
      \cline{2-5}
      ~                                   & $\mbox{10-shot}$                          & $\mbox{20-shot}$                          & $\mbox{10-shot}$                          & $\mbox{20-shot}$                          \\
      \midrule
      % \cline{1-11}
      Point-BERT~\cite{yu2022pointbert}   & 94.6{\scriptsize $\pm$3.6}                & 93.9{\scriptsize $\pm$3.1}                & 86.4{\scriptsize $\pm$5.4}                & 91.3{\scriptsize $\pm$4.6}                \\
      % \cline{1-11}
      MaskPoint~\cite{liu2022maskpoint}   & 95.0{\scriptsize $\pm$3.7}                & 97.2{\scriptsize $\pm$1.7}                & 91.4{\scriptsize $\pm$4.0}                & 92.7{\scriptsize $\pm$5.1}                \\
      MAE3D~\cite{jiang2023masked}        & 95.2{\scriptsize $\pm$3.1}                & 97.9{\scriptsize $\pm$1.6}                & 91.1{\scriptsize $\pm$4.6}                & \underline{95.3{\scriptsize $\pm$3.1}}    \\
      PointMAE~\cite{pang2022pointmae}    & 96.3{\scriptsize $\pm$2.5}                & 97.8{\scriptsize $\pm$1.8}                & 92.6{\scriptsize $\pm$4.1}                & 93.4{\scriptsize $\pm$3.5}                \\
      PointGame~\cite{liu2023pointgame}                   & 96.7{\scriptsize $\pm$2.7}                & 97.9{\scriptsize $\pm$1.5}                & \underline{92.9{\scriptsize $\pm$3.7}}    & 94.7{\scriptsize $\pm$2.6}                \\
      PointLGMask~\cite{tang2023point}                 & \textbf{97.4{\scriptsize $\pm$2.0}}       & 98.1{\scriptsize $\pm$1.4}                & 92.6{\scriptsize $\pm$4.3}                & 95.1{\scriptsize $\pm$3.4}                \\
      PointGPT-S~\cite{chen2023pointgpt}  & 96.8{\scriptsize $\pm$2.0}                & \underline{98.6{\scriptsize $\pm$1.1}}    & 92.6{\scriptsize $\pm$4.6}                & 95.2{\scriptsize $\pm$3.4}                \\
      PointM2AE~\cite{zhang2022pointm2ae} & 96.8{\scriptsize $\pm$1.8}                & 98.3{\scriptsize $\pm$1.4}                & 92.3{\scriptsize $\pm$4.5}                & 95.0{\scriptsize $\pm$3.0}                \\
      % \textbf{Ours}                       & \underline{97.0{\scriptsize $\pm$2.4}}    & 98.5{\scriptsize $\pm$1.3}                & \underline{93.9{\scriptsize $\pm$3.9}}    & \underline{95.6{\scriptsize $\pm$3.8}}    \\
      \textbf{Ours}                       & \underline{97.2{\scriptsize $\pm$2.3}}    & \textbf{98.7{\scriptsize $\pm$1.2}}       & \textbf{93.2{\scriptsize $\pm$3.4}}       & \textbf{95.6{\scriptsize $\pm$2.6}}       \\
      % \hline
      % \multicolumn{5}{l}{Methods using cross-modal information or extra training data}      
      \midrule
      % CorssNet~\cite{}                    & {\color{gray} 96.8{\scriptsize $\pm$2.3}} & {\color{gray} 98.0{\scriptsize $\pm$1.4}} & {\color{gray} 93.3{\scriptsize $\pm$4.0}} & {\color{gray} 95.6{\scriptsize $\pm$2.8}} 
      % \\
      InterMAE~\cite{liu2023inter}                    & {\color{gray} 95.3{\scriptsize $\pm$2.1}} & {\color{gray} 97.7{\scriptsize $\pm$1.4}} & {\color{gray} 91.2{\scriptsize $\pm$3.7}} & {\color{gray} 94.0{\scriptsize $\pm$3.8}} \\
      ACT~\cite{dong2023act}              & {\color{gray} 96.8{\scriptsize $\pm$2.3}} & {\color{gray} 98.0{\scriptsize $\pm$1.4}} & {\color{gray} 93.3{\scriptsize $\pm$4.0}} & {\color{gray} 95.6{\scriptsize $\pm$2.8}} \\
      I2P-MAE~\cite{zhang2023i2pmae}      & {\color{gray} 97.0{\scriptsize $\pm$1.8}} & {\color{gray} 98.3{\scriptsize $\pm$1.3}} & {\color{gray} 92.6{\scriptsize $\pm$5.0}} & {\color{gray} 95.5{\scriptsize $\pm$3.0}} \\
      ReCon~\cite{qi2023recon}            & {\color{gray} 97.3{\scriptsize $\pm$1.9}} & {\color{gray} 98.0{\scriptsize $\pm$1.4}} & {\color{gray} 93.3{\scriptsize $\pm$3.9}} & {\color{gray} 95.8{\scriptsize $\pm$3.0}} \\
      PointGPT-L~\cite{chen2023pointgpt}  & {\color{gray} 98.0{\scriptsize $\pm$1.9}} & {\color{gray} 99.0{\scriptsize $\pm$1.0}} & {\color{gray} 94.1{\scriptsize $\pm$3.3}} & {\color{gray} 96.1{\scriptsize $\pm$2.8}} \\
      \bottomrule
    \end{tabular}
    % \vspace{-1em}
  \end{center}
  % \vspace{-1.5em}
\end{table}
